Outage Duration in Poisson Networks and its Application to Erasure Codes

We derive the probability distribution of the link outage duration at a typical receiver in a wireless network with Poisson distributed interferers sending messages with slotted random access over a Rayleigh fading channel. This result is used to analyze the performance of random linear network coding, showing that there is an optimum code rate and that interference correlation affects the decoding probability and throughput.

==> eval.tex <==
\section{Evaluation}\label{sec:eval}



\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[xlabel={Interference correlation $\rho(I_1,I_2)$},ylabel={Expected success duration $\expect{S}$},ymin=0,ymax=40,xmin=0,xmax=0.25,grid=both,
legend style={at={(0.98,0.98)}, anchor=north east, font=\footnotesize},
legend cell align=left
]

\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=10]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.1$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=9]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.09$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=8]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.08$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=7]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.07$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=6]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.06$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=5]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.05$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=4]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.04$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=3]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.03$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=2]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.02$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=1]  {images/succdur_plam_new.txt};\addlegendentry{$\lambda p=0.01$}

\end{axis}
\end{tikzpicture}
\caption{Expected time between consecutive outages over interference correlation $\rho(I_1,I_2)=\frac{p}{2}$, for different $\lambda p$. Parameters are $\theta=1$, $\alpha=3$, and $r=1$.}\label{fig:succdur_lampe}
\end{figure}


\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[xlabel={Interference correlation $\rho(I_1,I_2)$},ylabel={Expected success duration $\expect{S}$},ymin=0,ymax=30,xmin=0,xmax=0.25,grid=both,
legend style={at={(0.98,0.98)}, anchor=north east, font=\footnotesize},
legend cell align=left
]

\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=10]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=1$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=9]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.9$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=8]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.8$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=7]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.7$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=6]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.6$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=5]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.5$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=4]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.4$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=3]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.3$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=2]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.2$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=1]  {images/succdur_lam_p.txt};\addlegendentry{$\lambda=0.1$}

\end{axis}
\end{tikzpicture}
\caption{Expected time between consecutive outages over interference correlation $\rho(I_1,I_2)=\frac{p}{2}$, for different $\lambda$. Parameters are $\theta=1$, $\alpha=3$, and $r=1$.}\label{fig:succdur_lam_p}
\end{figure}


\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[xlabel={Interference correlation $\rho(I_1,I_2)$},ylabel={Expected success duration $\expect{S}$},ymin=0,ymax=40,xmin=0,xmax=0.25,grid=both,
legend style={at={(0.02,0.98)}, anchor=north west, font=\footnotesize},
legend cell align=left
]

\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=21]  {images/succdur_theta.txt};\addlegendentry{$\theta=2$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=19]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.9$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=17]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.8$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=15]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.7$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=13]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.6$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=11]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.5$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=9]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.4$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=7]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.3$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=5]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.2$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=3]  {images/succdur_theta.txt};\addlegendentry{$\theta=1.1$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=1]  {images/succdur_theta.txt};\addlegendentry{$\theta=1$}

\end{axis}
\end{tikzpicture}
\caption{Expected time between consecutive outages over interference correlation $\rho(I_1,I_2)=\frac{p}{2}$, for different $\theta$. Parameters are $\lambda p=0.01$, $\alpha=3$, and $r=1$.}\label{fig:succdur_theta_p}
\end{figure}


\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[xlabel={Interference correlation $\rho(I_1,I_2)$},ylabel={Expected success duration $\expect{S}$},ymin=0,ymax=8,xmin=0,xmax=0.25,grid=both,
legend style={at={(0.98,0.98)}, anchor=north east, font=\footnotesize},
legend cell align=left
]

\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=21]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=2$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=19]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.9$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=17]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.8$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=15]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.7$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=13]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.6$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=11]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.5$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=9]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.4$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=7]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.3$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=5]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.2$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=3]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1.1$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=1]  {images/succdur_constlam_theta.txt};\addlegendentry{$\theta=1$}

\end{axis}
\end{tikzpicture}
\caption{Expected time between consecutive outages over interference correlation $\rho(I_1,I_2)=\frac{p}{2}$, for different $\theta$. Parameters are $\lambda=1$, $\alpha=3$, and $r=1$.}\label{fig:succdur_constlam_theta_p}
\end{figure}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[xlabel={Interference correlation $\rho(I_1,I_2)$},ylabel={Expected success duration $\expect{S}$},ymin=0,ymax=40,xmin=0,xmax=0.25,grid=both,
legend style={at={(0.02,0.98)}, anchor=north west, font=\footnotesize},
legend cell align=left
]

\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=10]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=3$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=9]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.9$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=8]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.8$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=7]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.7$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=6]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.6$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=5]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.5$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=4]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.4$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=3]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.3$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=2]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.2$}
\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=1]  {images/succdur_alpha.txt};\addlegendentry{$\alpha=2.1$}

\end{axis}
\end{tikzpicture}
\caption{Expected time between consecutive outages over interference correlation $\rho(I_1,I_2)=\frac{p}{2}$, for different $\theta$. Parameters are $\lambda p=0.01$, $\theta=1$, and $r=1$.}\label{fig:succdur_alpha_p}
\end{figure}

==> sir.tex <==
\section{Moments of the SIR}\label{sec:sir}
We calculate the $n$th moment of the SIR $\moment{n}$ based on its ccdf given by $\suc{1}(\theta)$ in~\eqref{eq:cdf}. This yields
\begin{eqnarray}
\moment{n}&=&n\int_0^\infty \theta^{n-1} \suc{1}(\theta)\dd \theta\\\nonumber
&=&\Gamma\left(\frac{n}{\delta}+1\right)\left(\frac{\plc}{2\sqrt{r\pi}p\lambda\csc(\delta\pi)}\right)^{\frac{n}{\delta}}\:,
\end{eqnarray}
where $\delta=\frac{2}{\alpha}$.

Next, in order to gain some further insights on the distribution of the SIR, we calculate the probabilities that the SIR is above it mean plus $k$ times its standard deviation and get
\begin{eqnarray}
\lefteqn{\mathbb{P}\big[\sir\geq\expect{\sir}+m\,\var{\sir}\big]=}\\\nonumber
&=&\mathrm{e}^{-\left(\Gamma\left(\frac{1}{\delta}+1\right)+k\sqrt{-\Gamma^2\left(\frac{1}{\delta}+1\right)+\Gamma(\alpha+1)}\right)^\delta}\:.
\end{eqnarray}
In the case of $k=1$, this expression simplifies to $\mathbb{P}\big[\sir\geq\expect{\sir}\big]=\mathrm{e}^{-\left(\Gamma\left(\frac{1}{\delta}+1\right)\right)^\delta}$.

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[xlabel={Path-loss exponent $\alpha$},ylabel={Probability $\mathbb{P}\big[\sir\geq\expect{\sir}+m\,\var{\sir}\big]$},ymin=0,ymax=0.4,xmin=2,xmax=10,grid=both,
ymode=log,
legend style={at={(0.98,0.98)}, anchor=north east, font=\footnotesize},
legend cell align=left
]

\addplot plot[color=black,densely dotted,no marks,style=thick]  table[x index=0,y index=1]  {images/sir_mom.txt};\addlegendentry{$k=0$}
\addplot plot[color=black,densely dashed,no marks,style=thick]  table[x index=0,y index=2]  {images/sir_mom.txt};\addlegendentry{$k=1$}
\addplot plot[color=black,dashdotted,no marks,style=thick]  table[x index=0,y index=3]  {images/sir_mom.txt};\addlegendentry{$k=2$}
\addplot plot[color=black,dotted,no marks,style=thick]  table[x index=0,y index=4]  {images/sir_mom.txt};\addlegendentry{$k=3$}
\addplot plot[color=black,dashed,no marks,style=thick]  table[x index=0,y index=5]  {images/sir_mom.txt};\addlegendentry{$k=4$}
\addplot plot[color=black,solid,no marks,style=thick]  table[x index=0,y index=6]  {images/sir_mom.txt};\addlegendentry{$k=5$}

\end{axis}
\end{tikzpicture}
\caption{Probability that the SIR exceeds its mean plus $k$ times its standard deviation.}\label{fig:sir-mom}
\end{figure}

Fig.~\ref{fig:sir-mom} shows a plot of these probabilities for different $k$ in dependence of $\alpha$.
There is a number of interesting things to notice:
First, the probability does solely depend on the path-loss exponent $\alpha$ and on $k$; hence, it is independent of all other network parameters. Hence, this result applies to a wide range of network scenarios.
Second, with increasing $\alpha$ all these probabilities decrease and in the limit for $\alpha\to\infty$, they vanish. Hence, in a scenario with high path-loss the probability of the SIR exceeding its mean can be arbitrarily small. The reason is that the skewness of the distribution increases with increasing $\alpha$, which also can be verified by analyzing the expression for the skewness, which approaches infinity for $\alpha\to\infty$.
Third, for $k\geq 3$ there is a maximum probability at some $\alpha>2$. This indicates the path-loss exponent $\alpha$ that is worst in terms of outage performance of the network. For lower $\alpha$, outage is lower due to a smaller signal attenuation, while for higher $\alpha$ outage is reduced due to a smaller interference.
Note that the decrease of the probability with increasing $k$ is due to the increasing bound for the SIR and hence trivial.

